Quadratic Funding and Matching Funds Requirements

In this paper we examine the mechanism proposed by Buterin, Hitzig, and Weyl (2019) for public goods financing, particularly regarding its matching funds requirements, related efficiency implications, and incentives for strategic behavior. Then, we use emerging evidence from Gitcoin Grants, to identify stylized facts in contribution giving and test our propositions. Because of its quadratic design, matching funds requirements scale rapidly, particularly by more numerous and equally contributed projects. As a result, matching funds are exhausted early in the funding rounds, and much space remains for social efficiency improvement. Empirically, there is also a tendency by contributors to give small amounts, scattered among multiple projects, which accelerates this process. Among other findings, we also identify a significant amount of reciprocal backing, which could be consistent with the kind of strategic behavior we discuss.

==> images/lambdap_ronda7.tex <==
\begin{tabular}{p{3.5cm} p{1.8cm} p{1.8cm} p{1.8cm}}
\toprule
  Category &  Projects &       Mean &  Std. Dev. \\
\midrule
      Dapp &      57.0 &  10.606044 &   4.670976 \\
 Community &      53.0 &   5.889136 &   2.612311 \\
     Infra &      36.0 &  10.160159 &   3.298251 \\
     Matic &      19.0 &   1.927277 &   0.105503 \\
\bottomrule
\end{tabular}


==> images/lambdap_ronda7y8.tex <==
\begin{tabular}{p{3.5cm} p{1.8cm} p{1.8cm} p{1.8cm}}
\toprule
  Category &  Projects &       Mean &  Std. Dev. \\
\midrule
      Dapp - Round 7&      57 &  10.6060 &   4.6709 \\
 Community - Round 7 &      53 &   5.8891 &   2.6123 \\
     Infra - Round 7&      36 &  10.1602 &   3.2982 \\
     Matic - Round 7&      19 &   1.9273 &   0.1055 \\
 Community - Round 8 &     133 &  25.1127 &  21.2072 \\
      Dapp - Round 8&     114 &  16.6023 &  11.7582 \\
     Infra - Round 8&      43 &  22.8302 &  10.3061 \\
 East-Asia - Round 8&      23 &  14.7344 &   5.3482 \\
   Liftoff - Round 8&       3 &   0.2325 &   0.0793 \\

\bottomrule
\end{tabular}


==> images/lambdap_ronda8.tex <==
\begin{tabular}{p{3.5cm} p{1.8cm} p{1.8cm} p{1.8cm}}
\toprule
  Category &  Projects &       Mean &  Std. Dev. \\
\midrule
 Community &     133.0 &  25.112710 &  21.207224 \\
      Dapp &     114.0 &  16.602305 &  11.758234 \\
     Infra &      43.0 &  22.830232 &  10.306175 \\
 East-Asia &      23.0 &  14.734401 &   5.348232 \\
   Liftoff &       3.0 &   0.232495 &   0.079374 \\
\bottomrule
\end{tabular}


==> images/reciprocal_percentages.tex <==
\begin{tabular}{p{3.5cm} p{2.5cm} p{2.5cm} p{2.5cm}}
\toprule
   Category &  Number of projects \% &  Number of projects- complement \% &  Reciprocal investments in other categories \% \\
\midrule
  Community &              33.49 &                         66.51 &                                      71.30 \\
  Dapp Tech &              33.49 &                         66.51 &                                      55.55 \\
 Infra Tech &              22.64 &                         77.36 &                                      76.00 \\
      Matic &              8.96 &                         91.04 &                                      20.51 \\
\bottomrule
\end{tabular}


==> images/regressions2dd.tex <==
\begin{tabular}{lp{2.5cm} p{2cm} p{2cm}}
\toprule
   Dependent: Sqrt(c) &        (1) &         (2) \\
\midrule
            Intercept &  1.7472*** &   1.9966*** \\
                      &   (0.0583) &    (0.4227) \\
        Category Dapp &     0.0261 &             \\
                      &   (0.0927) &             \\
  Category Infra Tech &  0.4674*** &             \\
                      &   (0.1261) &             \\
       Category Matic &  0.5608*** &             \\
                      &   (0.0651) &             \\
                 Post &  -0.1813** &  -0.2915*** \\
                      &   (0.0905) &    (0.0993) \\
                   DD &  1.1864*** &        -0.0 \\
                      &   (0.0606) &    (0.1558) \\
 Project Fixed Effect &         No &         Yes \\
       Number of obs. &       8650 &        8650 \\
               Adj-R2 &      0.004 &       0.031 \\
         F-statistic: &    1134.67 &     211.619 \\
   Prob (F-statistic) &          0 &           0 \\
\bottomrule
\end{tabular}


==> images/regressionsDD1.tex <==
\begin{tabular}{p{3.5cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm} }
\toprule
Dependent: Squared root of contribution &         (1) &         (2) &         (3) &         (4) \\
\midrule
                              Intercept &   1.9569*** &   2.0231*** &   1.8298*** &   1.8745*** \\
                                        &    (0.1388) &    (0.1497) &    (0.0907) &    (0.1133) \\
                          Category Dapp &      0.0223 &       0.037 &    1.083*** &    1.212*** \\
                                        &    (0.1347) &    (0.3231) &    (0.0748) &    (0.1966) \\
                    Category Infra Tech &    0.4735** &     -0.0332 &   1.3742*** &   0.9291*** \\
                                        &    (0.1885) &    (0.3815) &    (0.0706) &    (0.2561) \\
                         Category Matic &   0.7828*** &   0.7808*** &   1.5012*** &   1.5337*** \\
                                        &    (0.2274) &    (0.2716) &    (0.1579) &    (0.2228) \\
                                      t &  -0.0502*** &  -0.0641*** &  -0.0685*** &  -0.0843*** \\
                                        &     (0.018) &    (0.0221) &    (0.0177) &    (0.0222) \\
                                   Post &     -0.0703 &      0.0772 &       0.096 &       0.233 \\
                                        &    (0.4375) &    (0.3605) &    (0.4621) &    (0.3197) \\
                                Increased &    1.174*** &   1.2422*** &   0.3286*** &   0.3409*** \\
                                        &    (0.1376) &    (0.1972) &    (0.0749) &    (0.1205) \\
                                     Post*Increased &       0.329 &      0.1774 &      0.1923 &      0.0518 \\
                                        &    (0.4161) &    (0.3854) &    (0.4501) &    (0.3427) \\
                   Project Fixed Effect &          No &          No &         Yes &         Yes \\
                 Category linear trends &          No &         Yes &          No &         Yes \\
                         Number of obs. &        8650 &        8650 &        8650 &        8650 \\
                                 Adj-R2 &       0.005 &       0.006 &       0.033 &       0.033 \\
                           F-statistic: &     367.027 &     269.205 &      83.347 &      51.652 \\
                     Prob (F-statistic) &           0 &           0 &           0 &           0 \\
\bottomrule
\end{tabular}


==> images/regressionsDD2.tex <==
\begin{tabular}{p{3.5cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm} }
\toprule
Dependent: Squared root of contribution &        (1) &        (2) &        (3) &        (4) \\
\midrule
                              Intercept &  1.6811*** &  1.7579*** &  1.2939*** &   1.942*** \\
                                        &   (0.1205) &   (0.1773) &   (0.1168) &      (0.2) \\
                          Category Dapp &     0.0471 &     0.1197 &  1.6631*** &    1.14*** \\
                                        &   (0.2032) &   (0.2991) &    (0.077) &   (0.1285) \\
                    Category Infra Tech &   0.5425** &     0.1294 &   2.074*** &  0.8225*** \\
                                        &   (0.2628) &   (0.3194) &   (0.0573) &    (0.071) \\
                         Category Matic &  0.6343*** &   0.6205** &  1.3915*** &  2.2013*** \\
                                        &   (0.2101) &   (0.3005) &   (0.2031) &   (0.4045) \\
                                   Post &    -0.2649 &  -0.9059** &     0.1015 &    -1.0707 \\
                                        &   (0.5075) &   (0.4078) &    (0.622) &   (0.7055) \\
                                Increased &  1.0468*** &  1.1374*** &    -0.0975 &    -0.2593 \\
                                        &   (0.1553) &   (0.2587) &   (0.1299) &   (0.2349) \\
                                     Post*Increased &     0.0499 &     0.6756 &    -0.3232 &    1.3205* \\
                                        &    (0.514) &   (0.4872) &   (0.6202) &   (0.7242) \\
                   Project Fixed Effect &         No &         No &        Yes &        Yes \\
                            Data window &     2 days &     2 days &      1 day &      1 day \\
                         Number of obs. &       1856 &        856 &       1856 &        856 \\
                                 Adj-R2 &      0.005 &     -0.001 &      0.124 &      0.332 \\
                           F-statistic: &      201.9 &    160.929 &     100.18 &    290.313 \\
                     Prob (F-statistic) &          0 &          0 &          0 &          0 \\
\bottomrule
\end{tabular}


==> images/regressionsclose.tex <==
\begin{tabular}{lp{2.5cm} p{1.5cm} p{1.6cm} p{1.6cm} p{1.6cm} p{1.6cm} p{1.6cm}}
\toprule
   Dependent: Sqrt(c) &         (1) &        (2) &        (3) &         (4) &        (5) &        (6) \\
\midrule
            Intercept &   2.9336*** &  2.7292*** &  2.9127*** &   1.9966*** &  1.1873*** &  1.7064*** \\
                      &    (0.0996) &   (0.1655) &   (0.3068) &    (0.3929) &   (0.1446) &    (0.377) \\
        Category Dapp &      0.0261 &      0.047 &     0.1183 &    0.9406** &  1.6504*** &  1.3449*** \\
                      &    (0.0927) &   (0.1555) &   (0.2807) &    (0.4024) &   (0.2328) &   (0.4448) \\
  Category Infra Tech &   0.4674*** &   0.5424** &      0.127 &   1.2353*** &  2.0777*** &   0.8122** \\
                      &    (0.1261) &   (0.2129) &   (0.2903) &    (0.4433) &    (0.144) &   (0.3596) \\
       Category Matic &  -0.6256*** &  -0.4335** &  -0.7569** &    0.9406** &  1.6504*** &  1.3449*** \\
                      &    (0.1115) &    (0.202) &   (0.3303) &    (0.4216) &   (0.3798) &   (0.4736) \\
                 Post &   -0.1813** &     -0.217 &    -0.2567 &  -0.2915*** &    -0.2126 &     0.2262 \\
                      &    (0.0905) &   (0.1536) &   (0.2538) &    (0.0993) &   (0.1446) &   (0.1786) \\
 Project Fixed Effect &          No &         No &         No &         Yes &        Yes &        Yes \\
          Data window &    Complete &     2 days &      1 day &    Complete &     2 days &      1 day \\
       Number of obs. &        8650 &       1856 &        856 &        8650 &       1856 &        856 \\
               Adj-R2 &       0.004 &      0.006 &     -0.001 &       0.031 &      0.124 &      0.332 \\
         F-statistic: &       19.17 &       4.26 &      2.677 &     407.061 &     16.801 &     69.988 \\
   Prob (F-statistic) &           0 &      0.002 &      0.031 &           0 &          0 &          0 \\
\bottomrule
\end{tabular}


==> images/regressionsk.tex <==
\begin{tabular}{lp{2.5cm} p{2cm} p{2cm} p{2cm}}
\toprule
    Dependent: Sqrt(c) &         (1) &        (2) &         (3) \\
\midrule
             Intercept &   2.9098*** &  1.9893*** &   2.0299*** \\
                       &    (0.0885) &   (0.3983) &    (0.3907) \\
         Category Dapp &      0.1086 &   1.0488** &   1.1628*** \\
                       &    (0.1027) &   (0.4136) &    (0.4145) \\
   Category Infra Tech &   0.4987*** &  1.2687*** &    1.0134** \\
                       &    (0.1235) &   (0.4484) &    (0.4507) \\
        Category Matic &  -0.6979*** &   0.8435** &   1.1431*** \\
                       &    (0.1205) &   (0.4226) &    (0.4313) \\
                     $k$ &    -0.0186* &  -0.031*** &  -0.0678*** \\
                       &    (0.0097) &   (0.0104) &    (0.0235) \\
       $k$*Category Dapp &             &            &       0.023 \\
                       &             &            &    (0.0263) \\
$k$*Category Infra Tech &             &            &    0.0737** \\
                       &             &            &    (0.0329) \\
      $k$*Category Matic &             &            &  -0.4104*** \\
                       &             &            &     (0.147) \\
  Project Fixed Effect &          No &        Yes &         Yes \\
        Number of obs. &        8650 &       8650 &        8650 \\
                Adj-R2 &       0.004 &      0.031 &       0.033 \\
          F-statistic: &      19.005 &    515.592 &     8049.32 \\
    Prob (F-statistic) &           0 &          0 &           0 \\
\bottomrule
\end{tabular}


==> images/regressionsk_round8.tex <==
\begin{tabular}{p{3.5cm} p{1.8cm} p{1.8cm} p{1.8cm}}
\toprule
Dependent: Squared root of contribution &         (1) &         (2) &         (3) \\
\midrule
                              Intercept &   2.5803*** &   2.6311*** &   2.5979*** \\
                                        &    (0.2393) &    (0.6877) &    (0.6942) \\
                     Category Community &     0.4992* &    -1.3337* &     -1.224* \\
                                        &    (0.2913) &    (0.7236) &    (0.7289) \\
                          Category Dapp &     -0.1607 &   -1.6627** &    -1.682** \\
                                        &    (0.2449) &    (0.7088) &      (0.72) \\
                     Category East-Asia &  -0.6512*** &   -1.7452** &   -1.5168** \\
                                        &    (0.2434) &    (0.7134) &    (0.7219) \\
                         Category Infra &      0.0041 &   -1.6785** &  -1.9623*** \\
                                        &    (0.2484) &    (0.7234) &    (0.7407) \\
                       Category Liftoff &     -0.5247 &      -0.928 &     -1.0205 \\
                                        &    (0.4505) &    (0.6481) &    (0.6818) \\
                                      k &  -0.0094*** &  -0.0076*** &      0.0228 \\
                                        &     (0.002) &    (0.0016) &    (0.2082) \\
                   k*Category Community &             &             &     -0.0315 \\
                                        &             &             &    (0.2082) \\
                        k*Category Dapp &             &             &     -0.0285 \\
                                        &             &             &    (0.2082) \\
                   k*Category East-Asia &             &             &     -0.0484 \\
                                        &             &             &    (0.2083) \\
                       k*Category Infra &             &             &     -0.0182 \\
                                        &             &             &    (0.2083) \\
                     k*Category Liftoff &             &             &      5.8616 \\
                                        &             &             &    (6.0959) \\
                   Project Fixed Effect &          No &         Yes &         Yes \\
                         Number of obs. &       23693 &       23693 &       23693 \\
                                 Adj-R2 &       0.005 &       0.039 &        0.04 \\
                           F-statistic: &      21.547 &     256.122 &     161.302 \\
                     Prob (F-statistic) &           0 &           0 &           0 \\
\bottomrule
\end{tabular}


==> images/sum_stats1.tex <==
\begin{table}[]
\begin{tabular}{llcc}
 & \multicolumn{1}{c}{N} & Mean & Standard error \\
\textit{Dapp Tech category. projects: 93, contributors: 1104} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
ci & 1104 & 66.774 & 14.243 \\
sqrt_ci & 1104 & 4.366 & 0.208 \\
\textit{Infra Tech category. projects: 56, contributors: 613} &  &  &  \\
ci & 613 & 142.331 & 42.900 \\
sqrt_ci & 613 & 6.055 & 0.416 \\
\textit{Community category. projects: 82, contributors: 677} &  &  &  \\
ci & 677 & 67.601 & 10.599 \\
sqrt_ci & 677 & 5.234 & 0.244 \\
\textit{Matic category. projects: 19, contributors: 190} &  &  &  \\
ci & 190 & 19.270 & 3.767 \\
sqrt_ci & 190 & 3.551 & 0.188
\end{tabular}
\end{table}

==> images/sum_stats1b.tex <==
\begin{tabular}{p{6cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm}}
\toprule
 & N & Mean & Std. dev. & Std. error & Median \\
\midrule
\textit{All categories. projects: 249, contributors: 1234} &  &  &  & \\
$c_i$ & 8450 & 24.895 & 161.778 & 1.76 & 4.75 \\
$\sqrt{c_i}$ & 8450 & 2.829 & 4.112 & 0.04 & 2.179 \\
\textit{Dapp Tech category. projects: 93, contributors: 1105} & \textit{} & \textit{} &  &  \\
$c_i$ & 3802 & 19.407 & 120.596 & 1.956 & 3.64 \\
$\sqrt{c_i}$ & 3798 & 2.466 & 3.654 & 0.059 & 1.908\\
\textit{Infra Tech category. projects: 56, contributors: 613} & \textit{} & \textit{} &  &  \\
$c_i$ & 2220 & 39.301 & 247.737 & 5.258 & 4.75\\
$\sqrt{c_i}$ & 2220 & 3.370 & 5.287 & 0.112 & 2.179\\
\textit{Community category. projects: 82, contributors: 677} & \textit{} & \textit{} &  &  \\
$c_i$ & 2142 & 21.366 & 115.481 & 2.495 & 4.75\\
$\sqrt{c_i}$ & 2142 & 2.958 & 3.553 & 0.077 & 2.179\\
\textit{Matic category. projects: 19, contributors: 190} & \textit{} & \textit{} &  &  \\
$c_i$ & 345 & 10.613 & 39.070 & 2.103 & 3.3\\
$\sqrt{c_i}$ & 345 & 2.401 & 2.205 & 0.119 & 1.817\\
\bottomrule
\end{tabular}



==> images/sum_stats_round8.tex <==
\begin{tabular}{lccccc}
\toprule
Category & Variable & N & Mean & Std. Dev. & Median \\ \hline
All & $c_i$ & 18392 & 29.632 & 482.553 & 4.470 \\
\textit{(projects: 444 contributors:   4953)} & $\sqrt{c_i}$ & 18392 & 2.625 & 4.769 & 2.114 \\
Dapp & $c_i$ & 6317 & 19.466 & 379.871 & 3.800 \\
\textit{(projects: 182 contributors:   2608)} & $\sqrt{c_i}$ & 6317 & 2.385 & 3.712 & 1.949 \\
Community & $c_i$ & 7311 & 37.862 & 632.955 & 4.250 \\
\textit{(projects: 177 contributors:   2854)} & $\sqrt{c_i}$ & 7311 & 2.697 & 5.531 & 2.062 \\
Infra & $c_i$ & 4295 & 25.742 & 301.379 & 4.410 \\
\textit{(projects: 55 contributors:   1431)} & $\sqrt{c_i}$ & 4295 & 2.551 & 4.386 & 2.100 \\
East-Asia & $c_i$ & 1293 & 16.619 & 88.176 & 3.800 \\
\textit{(projects: 38 contributors:   811)} & $\sqrt{c_i}$ & 1293 & 2.662 & 3.088 & 1.949 \\
Lift-off & $c_i$ & 137 & 28.540 & 245.225 & 0.998 \\
\textit{(projects: 10 contributors:   119)} & $\sqrt{c_i}$ & 137 & 1.874 & 5.021 & 0.999 \\
Apollo & $c_i$ & 332 & 27.908 & 198.974 & 2.000 \\
\textit{(projects: 20 contributors:   287)} & $\sqrt{c_i}$ & 332 & 2.608 & 4.601 & 1.414 \\ \hline
\end{tabular}


==> images/sumstats1.tex <==

\begin{tabular}{ll}
Categories & 4 \\
Projects & 249 \\
Backers & 1234
\end{tabular}



==> tables/lambdap_ronda7.tex <==
\begin{tabular}{p{3.5cm} p{1.8cm} p{1.8cm} p{1.8cm}}
\toprule
  Category &  Projects &       Mean &  Std. Dev. \\
\midrule
      Dapp &      57.0 &  10.606044 &   4.670976 \\
 Community &      53.0 &   5.889136 &   2.612311 \\
     Infra &      36.0 &  10.160159 &   3.298251 \\
     Matic &      19.0 &   1.927277 &   0.105503 \\
\bottomrule
\end{tabular}


==> tables/lambdap_ronda8.tex <==
\begin{tabular}{p{3.5cm} p{1.8cm} p{1.8cm} p{1.8cm}}
\toprule
  Category &  Projects &       Mean &  Std. Dev. \\
\midrule
 Community &     133.0 &  25.112710 &  21.207224 \\
      Dapp &     114.0 &  16.602305 &  11.758234 \\
     Infra &      43.0 &  22.830232 &  10.306175 \\
 East-Asia &      23.0 &  14.734401 &   5.348232 \\
   Liftoff &       3.0 &   0.232495 &   0.079374 \\
\bottomrule
\end{tabular}


==> tables/regressions2dd.tex <==
\begin{tabular}{lp{2.5cm} p{2cm} p{2cm}}
\toprule
   Dependent: Sqrt(c) &        (1) &         (2) \\
\midrule
            Intercept &  1.7472*** &   1.9966*** \\
                      &   (0.0583) &    (0.4227) \\
        Category Dapp &     0.0261 &             \\
                      &   (0.0927) &             \\
  Category Infra Tech &  0.4674*** &             \\
                      &   (0.1261) &             \\
       Category Matic &  0.5608*** &             \\
                      &   (0.0651) &             \\
                 Post &  -0.1813** &  -0.2915*** \\
                      &   (0.0905) &    (0.0993) \\
                   DD &  1.1864*** &        -0.0 \\
                      &   (0.0606) &    (0.1558) \\
 Project Fixed Effect &         No &         Yes \\
       Number of obs. &       8650 &        8650 \\
               Adj-R2 &      0.004 &       0.031 \\
         F-statistic: &    1134.67 &     211.619 \\
   Prob (F-statistic) &          0 &           0 \\
\bottomrule
\end{tabular}


==> tables/regressionsclose.tex <==
\begin{tabular}{lp{2.5cm} p{1.5cm} p{1.6cm} p{1.6cm} p{1.6cm} p{1.6cm} p{1.6cm}}
\toprule
   Dependent: Sqrt(c) &         (1) &        (2) &        (3) &         (4) &        (5) &        (6) \\
\midrule
            Intercept &   2.9336*** &  2.7292*** &  2.9127*** &   1.9966*** &  1.1873*** &  1.7064*** \\
                      &    (0.0996) &   (0.1655) &   (0.3068) &    (0.3929) &   (0.1446) &    (0.377) \\
        Category Dapp &      0.0261 &      0.047 &     0.1183 &    0.9406** &  1.6504*** &  1.3449*** \\
                      &    (0.0927) &   (0.1555) &   (0.2807) &    (0.4024) &   (0.2328) &   (0.4448) \\
  Category Infra Tech &   0.4674*** &   0.5424** &      0.127 &   1.2353*** &  2.0777*** &   0.8122** \\
                      &    (0.1261) &   (0.2129) &   (0.2903) &    (0.4433) &    (0.144) &   (0.3596) \\
       Category Matic &  -0.6256*** &  -0.4335** &  -0.7569** &    0.9406** &  1.6504*** &  1.3449*** \\
                      &    (0.1115) &    (0.202) &   (0.3303) &    (0.4216) &   (0.3798) &   (0.4736) \\
                 Post &   -0.1813** &     -0.217 &    -0.2567 &  -0.2915*** &    -0.2126 &     0.2262 \\
                      &    (0.0905) &   (0.1536) &   (0.2538) &    (0.0993) &   (0.1446) &   (0.1786) \\
 Project Fixed Effect &          No &         No &         No &         Yes &        Yes &        Yes \\
          Data window &    Complete &     2 days &      1 day &    Complete &     2 days &      1 day \\
       Number of obs. &        8650 &       1856 &        856 &        8650 &       1856 &        856 \\
               Adj-R2 &       0.004 &      0.006 &     -0.001 &       0.031 &      0.124 &      0.332 \\
         F-statistic: &       19.17 &       4.26 &      2.677 &     407.061 &     16.801 &     69.988 \\
   Prob (F-statistic) &           0 &      0.002 &      0.031 &           0 &          0 &          0 \\
\bottomrule
\end{tabular}


==> tables/regressionsk_round8.tex <==
\begin{tabular}{p{3.5cm} p{1.8cm} p{1.8cm} p{1.8cm}}
\toprule
Dependent: Squared root of contribution &         (1) &         (2) &         (3) \\
\midrule
                              Intercept &   2.5803*** &   2.6311*** &   2.5979*** \\
                                        &    (0.2393) &    (0.6877) &    (0.6942) \\
                     Category Community &     0.4992* &    -1.3337* &     -1.224* \\
                                        &    (0.2913) &    (0.7236) &    (0.7289) \\
                          Category Dapp &     -0.1607 &   -1.6627** &    -1.682** \\
                                        &    (0.2449) &    (0.7088) &      (0.72) \\
                     Category East-Asia &  -0.6512*** &   -1.7452** &   -1.5168** \\
                                        &    (0.2434) &    (0.7134) &    (0.7219) \\
                         Category Infra &      0.0041 &   -1.6785** &  -1.9623*** \\
                                        &    (0.2484) &    (0.7234) &    (0.7407) \\
                       Category Liftoff &     -0.5247 &      -0.928 &     -1.0205 \\
                                        &    (0.4505) &    (0.6481) &    (0.6818) \\
                                      k &  -0.0094*** &  -0.0076*** &      0.0228 \\
                                        &     (0.002) &    (0.0016) &    (0.2082) \\
                   k*Category Community &             &             &     -0.0315 \\
                                        &             &             &    (0.2082) \\
                        k*Category Dapp &             &             &     -0.0285 \\
                                        &             &             &    (0.2082) \\
                   k*Category East-Asia &             &             &     -0.0484 \\
                                        &             &             &    (0.2083) \\
                       k*Category Infra &             &             &     -0.0182 \\
                                        &             &             &    (0.2083) \\
                     k*Category Liftoff &             &             &      5.8616 \\
                                        &             &             &    (6.0959) \\
                   Project Fixed Effect &          No &         Yes &         Yes \\
                         Number of obs. &       23693 &       23693 &       23693 \\
                                 Adj-R2 &       0.005 &       0.039 &        0.04 \\
                           F-statistic: &      21.547 &     256.122 &     161.302 \\
                     Prob (F-statistic) &           0 &           0 &           0 \\
\bottomrule
\end{tabular}


==> tables/sum_stats1.tex <==
\begin{table}[]
\begin{tabular}{llcc}
 & \multicolumn{1}{c}{N} & Mean & Standard error \\
\textit{Dapp Tech category. projects: 93, contributors: 1104} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
ci & 1104 & 66.774 & 14.243 \\
sqrt_ci & 1104 & 4.366 & 0.208 \\
\textit{Infra Tech category. projects: 56, contributors: 613} &  &  &  \\
ci & 613 & 142.331 & 42.900 \\
sqrt_ci & 613 & 6.055 & 0.416 \\
\textit{Community category. projects: 82, contributors: 677} &  &  &  \\
ci & 677 & 67.601 & 10.599 \\
sqrt_ci & 677 & 5.234 & 0.244 \\
\textit{Matic category. projects: 19, contributors: 190} &  &  &  \\
ci & 190 & 19.270 & 3.767 \\
sqrt_ci & 190 & 3.551 & 0.188
\end{tabular}
\end{table}

==> tables/sumstats1.tex <==

\begin{tabular}{ll}
Categories & 4 \\
Projects & 249 \\
Backers & 1234
\end{tabular}


